BACKDOORL: Backdoor Attack against Competitive Reinforcement Learning

Recent research has confirmed the feasibility of backdoor attacks in deep reinforcement learning (RL) systems. However, the existing attacks require the ability to arbitrarily modify an agent's observation, constraining the application scope to simple RL systems such as Atari games. In this paper, we migrate backdoor attacks to more complex RL systems involving multiple agents and explore the possibility of triggering the backdoor without directly manipulating the agent's observation. As a proof of concept, we demonstrate that an adversary agent can trigger the backdoor of the victim agent with its own action in two-player competitive RL systems. We prototype and evaluate BACKDOORL in four competitive environments. The results show that when the backdoor is activated, the winning rate of the victim drops by 17% to 37% compared to when not activated.

==> introduction_old.tex <==
\section{Introduction}

The backdoor attack is a novel attack vector aimed at deep learning models. In the world of computer security, a backdoor is a vulnerability in a system that allows unauthorized and unintended access when exploited. A backdoor attack involves an attacker unwillingly inserting a backdoor into victims' systems in order to have an access point to information or privileges they are not intended to have. Recently, backdoors have been successfully implemented in deep learning models, specifically heavily so in neural networks used for computer vision, making backdoor attacks a diverse threat to the world of computing. By either poisoning the training data or manipulating the inner weight of a model, an adversary can manage to insert a backdoor into the model that can be triggered by some special, attacker-specified inputs. 
%
For instance, a malicious attacker may inject a backdoor in the object-recognition model of a self-driving car system so that whenever a sticky note of specific shape is on the traffic sign, the model will fail to recognize it and thus lead to an accident as a result. \cite{gu} For these reasons, it is important to come up with feasible attack mechanisms before malicious adversaries in order to defend against them. 

While these backdoor attacks have been extensively studied in the context of computer vision, we desire to show that they are equally as implementable in the context of reinforcement learning. 
%
In this work, our goal is to migrate backdoor attacks to a competitive multi-agent scenario, where deep reinforcement learning agents are used, and creating a backdoor to be as evasive from detection as possible. 
%
Take for example a scenario such as a game called "Run to Goal", where each agent wants to be the first to run to its finish line. We want to insert a backdoor into one agent (the victim agent) so that when the other agent behaves normally, the victim agent will also behave normally, and when the other agent exhibits trigger behavior (the trigger agent), the victim agent will fail with high probability.

This attack is different from traditional backdoor attacks in deep learning because the traditional backdoor attack assumes that the attacker has full control over the input to the victim network; the trigger agent does not have the ability to directly modify the input (i.e. observation) to the victim agent because of the interactive nature of a multi-agent environment. Therefore, it needs to affect the next state of the game via its own behavior. Traditional backdoor attacks only need to trigger the victim network to output one wrong prediction, but in a competitive multi-agent setting, the trigger agent needs to lead the victim to output a series of wrong behaviors in order to prevent it from winning. In a competitive multi-agent setting, how do we design trigger and victim behavior in within different environments? One trivial solution may be to manually design the behavior (hardcode them in an agent and imitate the behavior using a network), however because there are so many different possible environments, it is very hard to manually design desired behaviors for every single one. Hardcoding for a specific environment also does not provide the opportunity to adapt the attack to brand new environments, therefore manual, hardcoded design is impractical since many new environments can be made.
Regardless of whether it is a single agent or multi-agent environment, deep reinforcement learning algorithms are notoriously hard to implement backdoor attacks in, as the state is constantly changing. Due to the constantly changing state of the game, the attacker must has to provide a pattern of malicious inputs as a function of time to get the victim to consequentially perform some chain of actions to have it end in failure.

In this paper, we propose BackdooRL, a stealthy novel attack to automatically generate a pair of victim and trigger agents without manually designing complex, noticeable triggers using Gu et al.'s BadNet \cite{gu} and adversarial training as building blocks. Our attack allows an agent who knows the backdoor "trigger action" to cause the opposing victim agent to fail at their command and thus win the game. The victim agent is a backdoored agent which, when observing the trigger action, fails the game automatically. This victim agent plays optimally when not faced with the trigger action. The attack maintains a stealthy appearance, making it much more evasive since it is difficult to discern. We also ensure that the failing behavior is produced quickly by the victim agent when viewing the trigger action, so that they lose as fast as possible to allow the other agent to win quickly and easily.

\lun{add contribution;}

